Towards Understanding the Role of Over-Parametrization in Generalization of Neural Networks

Despite existing work on ensuring generalization of neural networks in terms of scale sensitive complexity measures, such as norms, margin and sharpness, these complexity measures do not offer an explanation of why neural networks generalize better with over-parametrization. In this work we suggest a novel complexity measure based on unit-wise capacities resulting in a tighter generalization bound for two layer ReLU networks. Our capacity bound correlates with the behavior of test error with increasing network sizes, and could potentially explain the improvement in generalization with over-parametrization. We further present a matching lower bound for the Rademacher complexity that improves over previous capacity lower bounds for neural networks.

==> preliminaries.tex <==

Given $d,c,h>0$ and $\alpha,\beta\in \R_+$, we consider the following restricted set of parameters:
\begin{equation}\label{eq:param}
\calW=\left\{ (\vecV,\vecU) \mid \vecV\in \R^{c\times h},\vecU \in \R^{h\times d},\norm{\vecV}_{F}\leq \alpha,\norm{\vecU}_2\leq \beta, \forall_{j\in[h]},\vecu_i \in \calU_i\right\},
\end{equation}
where $\calU_i\subseteq \R^d$ is a subset of parameters for hidden unit $i$ and for simplicity of notation, we have dropped $d, c, h, \alpha,\beta$ from the notation $\calW$.
We now consider the following function class:
\begin{equation}\label{eq:class}
\calF_\calW=\left\{f(\vecx)=\vecV\left[\vecU \vecx\right]_+ \mid (\vecV,\vecU) \in \calW\right\}.
\end{equation}

Let $\ell_\gamma \circ \calH$ denotes the function class corresponding to the composition of loss function and functions in $\calH$. Then with probability $1-\delta$ over the choice of the training set, the following generalization bound holds for any $f \in \calH$  \citep[Theorem 3.1]{mohri2012foundations}:
\begin{equation}\label{eq:generalization}
L_{0}(f) \leq \hatL_\gamma(f) + 2\calR(\ell_\gamma \circ \calH) + \sqrt{\frac{\ln(2/\delta)}{2m}}.
\end{equation}
where $\calR(\calH)$ is the Rademacher complexity of a class $\calH$ of functions with respect to the input domain which is defined as:
\begin{equation}\label{eq:rademacher}
\calR(\calH) = \frac{1}{m}\sup_{\norm{\vecx_i}_2\leq 1 \atop{i\in[m]}}\E_{\xi \sim \left\{\pm 1\right\}^m} \left[\sup_{f\in \calH} \sum_{i=1}^m \xi_i f({x_i}) \right].
\end{equation}
Rademacher complexity captures the ability of functions in the function class to fit random noise. Similar generalization bounds can be given for empirical or expected Rademacher complexity. Since in practice these are within constant factor of each other, we chose the definition on unit ball domain to make the presentation simpler.

\paragraph{Unit complexity} Inspired by definition of Rademacher complexity, we define the unit complexity for each hidden unit in class $\calF_\calW$ as the Rademacher complexity of the class defined by that hidden unit, i.e. $\calR_{B}(\calF_{\calU_i})$ where $\calF_{\calU_i}=\{f(\vecx)=\inner{\vecu}{\vecx}\mid \vecu\in \calU_i\}$.


\begin{comment}
\paragraph{Unit impact} Unit impact captures the influence of a hidden unit on the output of the network. For example, if the outgoing weight of a hidden unit are all zero, that hidden unit cannot affect the output of the network and therefore has zero impact. We formally define the unit impacts $\{\calI_i\}_{i=1}^h$ such that for any $\vecz,\vecz'\in \R^h$ and any $(\vecV,\vecU)\in \calW$,
\begin{equation}
\norm{\vecV[\vecz]_+-\vecV[\vecz']_+}_2 \leq \sum_{i=1}^h \calI_i \abs{z_i-z'_i}
\end{equation}

Unit impact can be upper bounded by the magnitude of outgoing weights from the unit:
\begin{align*}
\norm{\vecV[\vecz]_+-\vecV[\vecz']_+}_2 &\leq\norm{\sum_{i=1}^h ([z_i]_+-[z'_i]_+)\vecv_i}_2\leq\sum_{i=1}^h\norm{([z_i]_+-[z'_i]_+)\vecv_i}_2\\
&\leq\sum_{i=1}^h\abs{[z_i]_+-[z'_i]_+}\norm{\vecv_i}_2\leq\sum_{i=1}^h\abs{z_i-z'_i}\norm{\vecv_i}_2\\
\end{align*}

\end{comment}




==> proofs_old.tex <==
\section{Old Proofs}



We will now present our key lemma that decomposes the complexity of a two layer ReLU network in terms of complexity of each layer. \TODO{Similar attempt was made at \cite{Fisher paper} Behnam: What paper is this?}.

\begin{lemma}[Rademacher decomposition lemma]\label{lem:decomposition}
	Given a training set $\calS=\{\vecx_i\}_{i=1}^m$ and $\gamma>0$, Rademacher complexity of the class $\calF_\calW$ defined in equations \eqref{eq:class} and \eqref{eq:param} is bounded as follows:
\begin{multline*}
m\calR_\calS(\ell_\gamma \circ \calF_\calW) \leq \frac{2}{\gamma}\sup_{\norm{\vecz_{i}}_2\leq \beta \norm{\vecx_i}_2}\E_{\vecxi_i \in \{\pm 1\}^{c}, i \in [m]} \left[\sup_{\norm{\vecV}_{F}\leq \alpha}\sum_{i=1}^{m} \inner{\vecxi_i}{\vecV\vecz_i}\right]\\	+ \frac{2\alpha}{\gamma}\sqrt{\sum_{j=1}^h \E_{\xi\in \{\pm 1\}^m}\left[\sum_{i=1}^{m} \sup_{\norm{\vecu_j-\vecu_j^0}\leq r_j}\xi_{i}\inner{\vecu_j}{\vecx_i}\right]^2}.	
\end{multline*}
\end{lemma}
\begin{proof}
We prove the following statement by induction on $t$:
\begin{align*}
& m\calR_\calS(\ell_\gamma \circ \calF_\calW)\\
& \leq \sup_{\norm{\vecz_{i}}\leq \beta \norm{\vecx_i}_2 \atop{ \norm{\vecV}_F\leq \alpha}}\E_{\vecxi_i \in \{\pm 1\}^{c}, i \in [m]} \left[\sup_{(\vecV,\vecU)\in \calW} \frac{2}{\gamma}\sum_{i=1}^{t-1} \left(\inner{\vecxi_i}{\vecV\vecz_i}+\xi_{i1}\sum_{j=1}^h \norm{\vecV_j}_2\inner{\vecu_j}{\vecx_i}\right)+\sum_{i=t}^m \xi_{i1}\ell_\gamma(\vecV[\vecU\vecx_i]_+,y_i)\right]\\
& = \sup_{\norm{\vecz_{i}}\leq \beta \norm{\vecx_i}_2 \atop{ \norm{\vecV}_F\leq \alpha}}\E_{\vecxi_i \in \{\pm 1\}^{c}, i \in [m]} \left[\sup_{(\vecV,\vecU)\in \calW} \xi_{t1}\ell_\gamma(\vecV[\vecU\vecx_t]_+,y_t) + \alpha_{\vecV,\vecU}\right],
\end{align*}
where for simplicity of the notation, we let $\alpha_{\vecV,\vecU}=\frac{2}{\gamma}\sum_{i=1}^{t-1} \left(\inner{\vecxi_i}{\vecV\vecz_i}+\xi_{i1}\sum_{j=1}^h \norm{\vecV_j}_2\inner{\vecu_j}{\vecx_i}\right)+\sum_{i=t+1}^m \xi_{i1}\ell_\gamma(\vecV[\vecU\vecx_i]_+,y_i)$. 
	
The above statement holds trivially for the base case of $t=1$. We now assume that it is true for any $t'\leq t$ and prove it is true for $t'=t+1$.
\begin{align}
m\calR_\calS(\ell_\gamma \circ \calF_\calW) &\leq  \sup_{\norm{\vecz_{i}}\leq \beta \norm{\vecx_i}_2 \atop{ \norm{\vecV}_F\leq \alpha}}\E_{\vecxi_i \in \{\pm 1\}^{c}, i \in [m]} \left[\sup_{(\vecV,\vecU)\in \calW} \xi_{t1}\ell_\gamma(\vecV[\vecU\vecx_t]_+,y_t) + \alpha_{\vecV,\vecU}\right] \nonumber \\
	&= \frac{1}{2} \sup_{\norm{\vecz_{i}}\leq \beta \norm{\vecx_i}_2 \atop{ \norm{\vecV}_F\leq \alpha}}\E_{\vecxi_i \in \{\pm 1\}^{c}, i \in [m]} \left[\sup_{(\vecV,\vecU), (\vecV',\vecU')\in \calW} \ell_\gamma(\vecV[\vecU\vecx_t]_+,y_t) - \ell_\gamma(\vecV'[\vecU'\vecx_t]_+,y_t) \right. \nonumber \\
	& \qquad \qquad + \left. \alpha_{\vecV,\vecU} +\alpha_{\vecV',\vecU'}\right] \nonumber \\
	&= \frac{1}{2} \sup_{\norm{\vecz_{i}}\leq \beta \norm{\vecx_i}_2 \atop{ \norm{\vecV}_F\leq \alpha}}\E_{\vecxi_i \in \{\pm 1\}^{c}, i \in [m]} \bigg[\sup_{(\vecV,\vecU),(\vecV',\vecU')\in \calW} \ell_\gamma(\vecV[\vecU\vecx_t]_+,y_t) -\ell_\gamma(\vecV'[\vecU\vecx_t]_+,y_t) \nonumber \\
	&\qquad \qquad + \ell_\gamma(\vecV'[\vecU\vecx_t]_+,y_t) -\ell_\gamma(\vecV'[\vecU'\vecx_t]_+,y_t) + \alpha_{\vecV,\vecU} +\alpha_{\vecV',\vecU'}\bigg] \nonumber \\
	&\leq \frac{1}{2} \sup_{\norm{\vecz_{i}}\leq \beta \norm{\vecx_i}_2 \atop{ \norm{\vecV}_F\leq \alpha}}\E_{\vecxi_i \in \{\pm 1\}^{c}, i \in [m]} \bigg[\sup_{(\vecV,\vecU),(\vecV',\vecU')\in \calW} \ell_\gamma(\vecV\vecz_t,y_t) -\ell_\gamma(\vecV'\vecz_t,y_t) \nonumber \\
	&\qquad \qquad + \ell_\gamma(\vecV'[\vecU\vecx_t]_+,y_t) -\ell_\gamma(\vecV'[\vecU'\vecx_t]_+,y_t) + \alpha_{\vecV,\vecU} +\alpha_{\vecV',\vecU'}\bigg]. \label{eq:proof_lemma1}
\end{align}	
The last inequality follows from $\|\vecU \vecx_t\|_2 \leq \beta \|\vecx_t\|_2$, for any $\vecx_t$, for $\vecU \in \calW$. 

For a given margin $\gamma > 0$, the loss will only change if the difference in function value is atleast $\frac{\gamma}{\sqrt{2}}$, as the prediction for two classes need to move a total distance of $\gamma$ to flip a label. $$ \ell_\gamma(\vecV\vecz_t,y_t) -\ell_\gamma(\vecV'\vecz_t,y_t) \leq  \frac{\norm{\vecV\vecz_t-\vecV'\vecz_t}_2}{ \sfrac{\gamma}{\sqrt{2}}} .$$ Similarly $$ \ell_\gamma(\vecV'[\vecU\vecx_t]_+,y_t) -\ell_\gamma(\vecV'[\vecU'\vecx_t]_+,y_t) \leq \frac{\sum_{j=1}^h \norm{\vecV_j}_2 \abs{\inner{\vecu_j}{\vecx_t} -\inner{\vecu'_j}{\vecx_t}}}{\sfrac{\gamma}{\sqrt{2}}}.$$ Here $\vecV_j$ is the $j$th row of $V$. Substituting the above two inequalities in equation \ref{eq:proof_lemma1} gives us,	
\begin{align*}	
& m\calR_\calS(\ell_\gamma \circ \calF_\calW) \\ & \leq \frac{1}{2} \sup_{\norm{\vecz_{i}}\leq \beta \norm{\vecx_i}_2 \atop{ \norm{\vecV}_F\leq \alpha}}\E_{\vecxi_i \in \{\pm 1\}^{c}, i \in [m]} \bigg[\sup_{(\vecV,\vecU),(\vecV',\vecU')\in \calW} \frac{\sqrt{2}}{\gamma}\left(\norm{\vecV\vecz_t-\vecV'\vecz_t}_2 + \sum_{j=1}^h\norm{\vecV_j}_2 \abs{\inner{\vecu_j}{\vecx_t} -\inner{\vecu'_j}{\vecx_t}}\right)\\
& \qquad \qquad  + \alpha_{\vecV,\vecU} +\alpha_{\vecV',\vecU'}\bigg]\\
& \stackrel{(i)}{\leq} \sup_{\norm{\vecz_{i}}\leq \beta \norm{\vecx_i}_2 \atop{ \norm{\vecV}_F\leq \alpha}}\E_{\vecxi_i \in \{\pm 1\}^{c}, i \in [m]} \bigg[\sup_{(\vecV,\vecU)\in \calW} \frac{2}{\gamma}\left(\inner{\vecxi_t}{\vecV\vecz_t}+\xi_{t1}\sum_{j=1}^h\norm{\vecV_j}\inner{\vecu_j}{\vecx_t}\right)\\
& \qquad \qquad + \alpha_{\vecV,\vecU} +\alpha_{\vecV',\vecU'}\bigg].
\end{align*}
$(i)$ follows from Lemma \ref{lem:contraction}.	This completes the induction proof. 

Hence the induction step at $t=m$ gives us:
\begin{align*}
& m\calR_\calS(\ell_\gamma \circ \calF_\calW) \\ &\leq  \frac{2}{\gamma} \sup_{\norm{\vecz_{i}}\leq \beta \norm{\vecx_i}_2 \atop{ \norm{\vecV}_F\leq \alpha}}\E_{\vecxi_i \in \{\pm 1\}^{c}, i \in [m]} \left[\sup_{(\vecV,\vecU)\in \calW}\sum_{i=1}^{m} \left( \inner{\vecxi_i}{\vecV\vecz_i}+\xi_{i1}\sum_{j=1}^h\norm{\vecV_j}_2 \inner{\vecu_j}{\vecx_i} \right) \right]\\
	&\leq  \frac{2}{\gamma} \sup_{\norm{\vecz_{i}}\leq \beta \norm{\vecx_i}_2 \atop{ \norm{\vecV}_F\leq \alpha}}\left(\E_{\vecxi_i \in \{\pm 1\}^{c}, i \in [m]} \left[\sup_{\norm{\vecV}_F\leq \alpha}\sum_{i=1}^{m} \inner{\vecxi_i}{\vecV\vecz_i}\right]+   \sum_{j=1}^h \norm{\vecV_j}_2 \E_{\xi\in \{\pm 1\}^m}\left[\sum_{i=1}^{m} \sup_{\norm{\vecu_j-\vecu_j^0}\leq r_i}  \xi_{i}\inner{\vecu_j}{\vecx_i}\right]\right)\\
		&\leq \frac{2}{\gamma}\sup_{\norm{\vecz_{i}}_2\leq \beta \norm{\vecx_i}_2 \atop{ \norm{\vecV}_F\leq \alpha} }\E_{\vecxi_i \in \{\pm 1\}^{c}, i \in [m]} \left[\sup_{\norm{\vecV}_{F}\leq \alpha}\sum_{i=1}^{m} \inner{\vecxi_i}{\vecV\vecz_i}\right]+ \frac{2}{\gamma}\norm{\vecV}_F \sqrt{\sum_{j=1}^h \E_{\xi\in \{\pm 1\}^m}\left[\sum_{i=1}^{m}\sup_{\norm{\vecu_j-\vecu_j^0}\leq r_j}\xi_{i}\inner{\vecu_j}{\vecx_i}\right]^2}\\
	&\leq \frac{2}{\gamma}\sup_{\norm{\vecz_{i}}_2\leq \beta \norm{\vecx_i}_2}\E_{\vecxi_i \in \{\pm 1\}^{c}, i \in [m]} \left[\sup_{\norm{\vecV}_{F}\leq \alpha}\sum_{i=1}^{m} \inner{\vecxi_i}{\vecV\vecz_i}\right]+ \frac{2\alpha}{\gamma}\sqrt{\sum_{j=1}^h \E_{\xi\in \{\pm 1\}^m}\left[\sum_{i=1}^{m}\sup_{\norm{\vecu_j-\vecu_j^0}\leq r_j}\xi_{i}\inner{\vecu_j}{\vecx_i}\right]^2}.
\end{align*} The last inequality follows from using the Cauchy-Schwarz inequality.
\end{proof}

\begin{theorem}\label{thm:generalization1}
For any $\gamma>0$ and $\delta\in(0,1)$, with probability $1-\delta$ over the choice of the training set $\calS=\{\vecx_i\}_{i=1}^m$, for any function $f$ in class $\calF_\calW$ defined in equations \eqref{eq:class} and \eqref{eq:param}, the generalization error is bounded as follows:
\begin{align*}
L_{0}(f) &\leq \hatL_\gamma(f) + \frac{4 \alpha\left(\beta \sqrt{c}+\norm{r}_2\right)\norm{\vecX}_F}{\gamma m }+ 3\sqrt{\frac{\ln(2/\delta)}{2m}}\\
&=\hatL_\gamma(f) + \frac{4 \alpha\left(\beta \sqrt{c}+\norm{\vecr}_2\right)\sqrt{\frac{1}{m}\sum_{i=1}^m\norm{\vecx_i}_2^2}}{\gamma \sqrt{m} }+ 3\sqrt{\frac{\ln(2/\delta)}{2m}}.
\end{align*}
\end{theorem}
This result assumes the knowledge of the norms of the network parameters $\alpha, \beta$ and $\vecr$. We will see how to get around this assumption using covering arguments in the proof of Theorem \ref{thm:generalization2}.

\begin{proof}
We prove this theorem by substituting the Rademacher complexity bound from Lemma \ref{lem:decomposition} in equation \eqref{eq:generalization}.

From Lemma \ref{lem:decomposition} we have \begin{multline*}
m\calR_\calS(\ell_\gamma \circ \calF_\calW) \leq \frac{2}{\gamma}\sup_{\norm{\vecz_{i}}_2\leq \beta \norm{\vecx_i}_2}\E_{\vecxi_i \in \{\pm 1\}^{c}, i \in [m]} \left[\sup_{\norm{\vecV}_{F}\leq \alpha}\sum_{i=1}^{m} \inner{\vecxi_i}{\vecV\vecz_i}\right]\\	+ \frac{2\alpha}{\gamma}\sqrt{\sum_{j=1}^h \E_{\xi\in \{\pm 1\}^m}\left[\sum_{i=1}^{m} \sup_{\norm{\vecu_j-\vecu_j^0}\leq r_j}\xi_{i}\inner{\vecu_j}{\vecx_i}\right]^2}.	
\end{multline*}
Bounding the inner product using Lemma \ref{lem:contraction} gives us, 
\begin{align*}
& m\calR_\calS(\ell_\gamma \circ \calF_\calW) \\ 
& \leq \frac{2}{\gamma}\sup_{\norm{\vecz_{i}}_2\leq \beta \norm{\vecx_i}_2}\E_{\vecxi_i \in \{\pm 1\}^{c}, i \in [m]} \left[\sup_{\norm{\vecV}_{F}\leq \alpha}\sum_{i=1}^{m} \inner{\vecxi_i}{\vecV\vecz_i}\right]	\\ 
& \qquad \qquad + \frac{2\alpha}{\gamma}\sqrt{\sum_{j=1}^h \E_{\xi\in \{\pm 1\}^m}\left[\sum_{i=1}^{m} \sup_{\norm{\vecu_j-\vecu_j^0}\leq r_j}\xi_{i}\inner{\vecu_j}{\vecx_i}\right]^2}	\\
& \leq \frac{2}{\gamma} \sqrt{c} \alpha \beta \norm{X}_F  + \frac{2\alpha}{\gamma}\sqrt{\sum_{j=1}^h r_j^2 \norm{X}_F^2 } \\
&= 	\frac{2}{\gamma} \alpha \left( \sqrt{c}  \beta   +  \sqrt{\sum_{j=1}^h r_j^2} \right) \norm{X}_F.
\end{align*}
Finally substituting the above Rademacher complexity bound in equation \eqref{eq:generalization} gives the result. 
\end{proof}


